AttentionFlow: Visualising Influence in Networks of Time Series

The collective attention on online items such as web pages, search terms, and videos reflects trends that are of social, cultural, and economic interest. Moreover, attention trends of different items exhibit mutual influence via mechanisms such as hyperlinks or recommendations. Many visualisation tools exist for time series, network evolution, or network influence; however, few systems connect all three. In this work, we present AttentionFlow, a new system to visualise networks of time series and the dynamic influence they have on one another. Centred around an ego node, our system simultaneously presents the time series on each node using two visual encodings: a tree ring for an overview and a line chart for details. AttentionFlow supports interactions such as overlaying time series of influence and filtering neighbours by time or flux. We demonstrate AttentionFlow using two real-world datasets, VevoMusic and WikiTraffic. We show that attention spikes in songs can be explained by external events such as major awards, or changes in the network such as the release of a new song. Separate case studies also demonstrate how an artist's influence changes over their career, and that correlated Wikipedia traffic is driven by cultural interests. More broadly, AttentionFlow can be generalised to visualise networks of time series on physical infrastructures such as road networks, or natural phenomena such as weather and geological measurements.

==> sections/related.tex <==
%!TEX root = ../main.tex

% ====================================================
\section{Related work}
\label{sec:related}

% This section reviews the techniques for visualising trends in temporal data, flows among graph entities, and evolution of ego networks.

% AttentionFlow: 1. visualising temporal trends in 2 visual encodings (line chart and tree ring), 2. evolution of ego network structure, and 3. the dynamic influence flows

% can do 1 but not 2, 3: multiple time series visualisations, e.g., Clustervision
% can do 2 but not 1, 3: dynamic ego network, e.g., see survey from Utah
% can do 3 but not 1, 2: sankey diagram, e.g., netflower, meanwhile sankey also fails to reveal the dynamic flows
% can do 1, 2 but not 3: Growth ring maps
% can do 1, 3 but not 2: IdeaFlow
% can do 2, 3 but not 1: EgoNetCloud, Eiffel, Influence flower, sabrina
% can do 1, 2, 3: AttentionFlow

% Clustervision: merely a unsupervised way to display multiple time series
% Growth ring maps: visualising temporal trends and network structure but not the network evolution
% IdeaFlow: visualising flow pathway but no network structure, nor network evolution
% EgoNetCloud: visualising the dynamic changes of the alters in an ego network structure, but not showing the temporal trends of the alters, this makes it lack the capability to identify correlated trends for 2 nodes.
% Eiffel: visualising the propagation path, but does not align it along time axis, thus fail to tell the story of how an entity progressively influences other entities over time
% Influence flower: no temporal view, thus unable to identify correlated temporal trends
% netflower: sankey diagram does not show the temporal influence change.
% sabrina: no time series views, unable to compare multiple edges and identify trends.

% ====================================================
\header{Characterising temporal patterns.}
A line chart is the most common way to visualise
a time series, but it lacks the
scalability to present many of them at once.
To address this, some works have developed techniques to stack\cite{havre2000themeriver} and cluster\cite{kwon2017clustervision} multiple time series.
% and cluster similar trends into distinct partitions.
% Clustervision\cite{kwon2017clustervision} uses an unsupervised method to group similar temporal patterns into distinct partitions.
Other works encode each series into a separate visual element.
% and present multiple elements as a network.
Bak et al.\cite{bak2009spatiotemporal} proposed a framework called Growth Ring Maps for spatiotemporal analysis.
They encoded a sensor's temporal records into a density circle and then placed multiple circles over the spatial dimension.
% Tree-ring visualisation is used to represent temporal evolution.
In a similar vein, Cruz et al.\cite{cruz2018process} introduced the tree ring visualisation to represent the immigrant population growth in the US.
% Other encodings for visualising a time series as a node include radial chart and circular heatmap.
Adnan et al.\cite{adnan2016investigating} evaluated the user perceptions of different time series visualisations.
% including radial chart and circular heatmap.
Their results suggest that colour encoding is the most effective presentation to recognise temporal trends.

In our work, \toolname adopts both the tree ring to provide a summary of the temporal pattern,
% how the collective attention on an entity is evolving over time.
and the line chart to highlight the correlation between two time series.

we adopt tree rings to present summaries, and use time series to present details and highlight correlation between time series
In our work, \toolname uses a tree-ring visualisation to provide a summary of
how user attention on an entity is distributed over time.
the attention time series attracted to an entity, in which different colours represent the attention intensity.
YouTube video (see \autoref{fig:nodegradient}).
We discretise the radius by calendar years and paint each year with different colour gradients.
This allows us to quickly compare the temporal trends across multiple entities and identify concurrent spikes.

\header{Influence visualisation.}
% Visualising flows in the network is another relevant area.
IdeaFlow\cite{wang2016ideas} visualises how ideas flow within and across multiple social groups by modelling the lead-lag relationships in text clusters.
% The volume of flows are often considered as quantifiable influences between two network entities.
Situ\cite{goodall2018situ} combined flow visualisation and anomaly detection to identify agents with suspicious network traffic.
In citation analysis, Shin et al.\cite{shin2019influence} proposed a flower-like metaphor for visualising the influence profile of academic entities.
Using an ego network, they presented the influence across different types of entities (e.g. authors, venues, or fields) throughout a scholar's scientific career.
Huang et al.\cite{huang2019eiffel} used a graph summarisation algorithm to compose the flow map of a paper's influence trajectory.
In financial systems, netflower\cite{stoiber2019netflower} adopts a Sankey diagram to visualise the monetary flow between government institutions and media outlets.
Nevertheless, Sankey diagrams are often not designed to demonstrate temporal changes.
The Sabrina system\cite{arleo2019sabrina} extends the flow map to three dimensions to map the relations between spatial entities.


Some of the existing visual analytics systems do not consider the temporal trends of entities\cite{arleo2019sabrina,goodall2018situ}, while others do not reveal the dynamic structural changes\cite{wang2016ideas,shin2019influence,huang2019eiffel,stoiber2019netflower}.
In contrast, our system simultaneously presents a trend view for identifying correlated spikes, and a network view for capturing the dynamic influence flows.
presents two views simultaneously: a trend view that provides fine granularity time series to identify concurrent spikes, and a network view that captures the dynamic flow in the dynamic ego networks.

But the temporal influence networks can only be compared by generating multiple snapshots over different eras.

\header{Visualisation of dynamic ego networks.}
% dynamic networks
% Visualising dynamic multivariate graph is challenging [...]
Beck et al.\cite{beck2014state} categorised dynamic graph visualisation techniques into animation and timeline approaches.
% Beck et al.\cite{beck2014state} surveyed the dynamic graph visualisation techniques.
% The authors divide techniques into animation and timeline according to how time is represented.
The same categorisation can be applied to ego networks.
% However, ego networks mainly focus on the characteristics of the ego and its relationship with the connected alters, rather than the topological overview for the entire network. 
Many studies choose the timeline approach.
% for visually highlighting the changes in the relationship in dynamic ego networks.
EgoSlider\cite{wu2015egoslider} uses a series of juxtaposed glyphs for visualising the network evolution of both the ego and the alters.
% Separate timeline network is used for tracking the changes in alters.
EgoLines\cite{zhao2016egolines} uses a subway map metaphor to visualise an author's collaboration trajectory over the years.
In these visualisations, the ego is divided into multiple glyphs or networks representing time slices which are defined by the relations with the surrounding alters. 
%
While the traditional node-edge layout can only represent a single network snapshot at a time, a number of efforts have been made to embed the timelines of nodes or edges in the ego networks.
% Reitz\cite{reitz2010framework} proposed a framework of using different colours to indicate the time evolution of times and changes in edge weights.
% Farrugia et al. \cite{farrugia2011exploring} introduced a metaphor of tree ring to reveal the temporal network evolution of an ego node.
% Other works embed timeline to ego node instead of edges.
Shi et al.\cite{shi2014d15} introduced central trend glyphs to represent the temporal changes in the ego node.
EgoNetCloud\cite{liu2015egonetcloud} presents the alters and their evolving relations along with the temporal trend of the ego.
Both works visualise the ego as a continuous trend, but the relationships between the ego and the alters are discrete based on when the links are formed.
This results in either multiple edges between the ego and the alters\cite{shi2014d15}, or duplicate alters across different time slices\cite{liu2015egonetcloud}. 
%

% Our \toolname system proposes a technique to interactively visualise the relationship changes between the ego and the alters while keeping the continuous trend of the ego as an anchor component.

Our \toolname system proposes a technique to overcome the limitations of the traditional node-link layout by interactively visualising the relationship changes between the ego and the alters while keeping the continuous trend of the ego as an anchor component.

